Multi-class Network Intrusion Detection with Class Imbalance via LSTM & SMOTE

Monitoring network traffic to maintain the quality of service (QoS) and to detect network intrusions in a timely and efficient manner is essential. As network traffic is sequential, recurrent neural networks (RNNs) such as long short-term memory (LSTM) are suitable for building network intrusion detection systems. However, in the case of a few dataset examples of the rare attack types, even these networks perform poorly. This paper proposes to use oversampling techniques along with appropriate loss functions to handle class imbalance for the detection of various types of network intrusions. Our deep learning model employs LSTM with fully connected layers to perform multi-class classification of network attacks. We enhance the representation of minority classes: i) through the application of the Synthetic Minority Over-sampling Technique (SMOTE), and ii) by employing categorical focal cross-entropy loss to apply a focal factor to down-weight examples of the majority classes and focus more on hard examples of the minority classes. Extensive experiments on KDD99 and CICIDS2017 datasets show promising results in detecting network intrusions (with many rare attack types, e.g., Probe, R2L, DDoS, PortScan, etc.).

==> section_lstm_eqns_cfcl.tex <==

\subsection{ Long Short Term Memory (LSTM) model}
A variety of RNN architectures are proposed for learning long-term dependencies to handle sequential data. LSTM, a variant of RNN, can effectively handle the dependency issues of long sequences due to its cell processor structure, which includes data operations for input, forget, and output gates to control the network \cite{hochreiter1997long}. 
%
\begin{align}
f_t &= \sigma(W_f \cdot [h_{t-1}, x_t] + b_f)  \label{lstm_eqn1} \\
i_t &= \sigma(W_i \cdot [h_{t-1}, x_t] + b_i)  \label{lstm_eqn2} \\
\tilde{C}_t &= \tanh(W_C \cdot [h_{t-1}, x_t] + b_c) \label{lstm_eqn3} \\
C_t &= f_t \odot C_{t-1} + i_t \odot \tilde{C}_t  \label{lstm_eqn4} \\
o_t &= \sigma(W_o \cdot [h_{t-1}, x_t] + b_o)  \label{lstm_eqn5} \\
h_t &= o_t \odot \tanh(C_t)  \label{lstm_eqn6} 
\end{align}
where, 

\begin{itemize}
  \item	$f_t$ is the forget gate output,
  \item	$i_t$ is the input gate output,
  \item	$\tilde{C}_t$  is the candidate cell state,
  \item   $ C_t $  is the cell state,
  \item   $ o_t$ is the output gate output,
  \item   $ h_t$ is the hidden state,
  \item   $ x_t$ is the input at time step 
  \item   $h_{t-1} $  is the hidden state from the previous time step,
  \item   $\sigma $ is the sigmoid activation function,
  \item   $\odot$ represents element-wise multiplication,
  \item  $W_f, b_f, W_i, b_i, W_C, b_C, W_o$, \text{and} $b_o$ are the weight matrices and bias terms.
\end{itemize}

The LSTM layer equations describe the forward pass of an LSTM layer over a sequence of time steps. For zero initial states:
  %
\begin{align*}\label{eqn_lstm_states}
h_0 &= \mathbf{0} \quad \text{(initial hidden state)} \\
C_0 &= \mathbf{0} \quad \text{(initial cell state)} \\
\text{for } t &= 1, 2, \ldots, T: \\
\quad h_t, C_t &= \text{LSTM\_Cell}(h_{t-1}, C_{t-1}, x_t),
\end{align*}
%
where,
\begin{itemize}
  \item $h_o$ and $C_o$ are the initial hidden state and cell state,
   \item $T$ is the number of time steps,
    \item $x_t$ is the input at timestep, 
    \item $h_t$ and $C_t$ are the updated hidden state and cell state at timestep $t$,
    \item $\text{LSTM\_Cell}$ represents the LSTM cell equations \ref{lstm_eqn1} - \ref{lstm_eqn6} .
\end{itemize}

 \textbf{Forget Gate Output} ($f_t$):
It decides what to retain or forget from the previous cell state $C_{t-1}$. It's determined by a Sigmoid activation of a weighted combination of $h_{t-1}$ and $x_t$, mapping values to [0, 1]. A value of 0 means "forget completely," and 1 means "remember fully."

\textbf{Input Gate Output} ($i_t$):
It determines what new information to store in the cell state. Similar to the forget gate, it's computed using a Sigmoid activation of a weighted combination of $h_{t-1}$ and $x_t$. This activation decides which values from the candidate cell state $\tilde{C}_t$ to add to the cell state $C_t$.

\textbf{Candidate Cell State} ($\tilde{C}_t$):
It represents new information that can be added to the cell state. It's calculated by applying the hyperbolic tangent (tanh) activation to a weighted combination of $h{t-1}$ and $x_t$, squashing values to [-1, 1].

\textbf{Cell State Update} ($C_t$):
It combines the previous cell state $C_{t-1}$ and the new candidate cell state $\tilde{C}t$ based on the forget gate $f_t$ and the input gate $i_t$, using element-wise multiplication ($\odot$). If $f_t$ is close to 1, corresponding components of $C{t-1}$ are retained. If $i_t$ is close to 1, corresponding components of $\tilde{C}_t$ are added to $C_t$.

\textbf{Output Gate Output} ($o_t$):
It determines what information from the updated cell state $C_t$ should be passed to the current hidden state $h_t$. It computes a Sigmoid activation of a weighted combination of $h_{t-1}$ and $x_t$. The Sigmoid activation scales the values in $C_t$ selectively.

\textbf{Hidden State Update} ($h_t$):
It is computed as the element-wise multiplication ($\odot$) of the output gate $o_t$ and the hyperbolic tangent (tanh) of the updated cell state $C_t$. This captures relevant information passed to the next time step.


The final layer of the LSTM network is a fully connected layer with the same number of neurons as the number of attack classes. It allows us to effectively process the temporal information present in the flow data and accurately classify the different types of network attacks.




==> section_table_draft.tex <==

\begin{table*}[htbp]
\centering
\caption{Comparison of the proposed method with other methods.}\label{comparison_cicids2017_table}
\resizebox{0.9\textwidth}{!}{%
\begin{tabular}{|c|c|c|c|c|c|c|c|c|c|c|c|c|c|}   
\hline
\multirow{2}{*}{\textbf{Label}} & \multicolumn{4}{c|}{\textbf{LSTM \cite{boukhalfa2020lstm}}} & \multicolumn{4}{c|}{\textbf{CNN + LSTM}\cite{sun2020dl}} & \multicolumn{4}{m{3cm}|}{\textbf{LSTM + Focal Loss + SMOTE (Proposed)}} \\
\cline{2-13}
 & ACC & TPR & PPV & F1 & ACC & TPR & PPV & F1 & ACC & TPR & PPV & F1 \\
\hline
BENIGN & 0.97 & 0.97 & 0.97 & 0.97 & 0.99 & 0.97 & 0.99 & 0.98 & 0.96 & 0.96 & 0.96 & 0.96 \\
Bot & 1.00 & 0.01 & 0.86 & 0.02 & 1.00 & 0.01 & 0.86 & 0.02 & 0.99 & 0.98 & 0.41 & 0.58 \\
Brute Force & 1.00 & 0.99 & 0.91 & 0.95 & 1.00 & 0.99 & 0.91 & 0.95 & 1.00 & 1.00 & 0.85 & 0.91 \\
DDoS & 1.00 & 1.00 & 1.00 & 1.00 & 1.00 & 1.00 & 1.00 & 1.00 & 1.00 & 1.00 & 0.98 & 0.99 \\
DoS & 1.00 & 1.00 & 0.99 & 0.99 & 1.00 & 1.00 & 0.99 & 0.99 & 1.00 & 1.00 & 0.96 & 0.98 \\
Heartbleed & 1.00 & 1.00 & 1.00 & 1.00 & 1.00 & 1.00 & 1.00 & 1.00 & 1.00 & 1.00 & 1.00 & 1.00 \\
Infiltration & 1.00 & 0.30 & 0.26 & 0.00 & 1.00 & 0.97 & 0.96 & 0.96 & 1.00 & 0.89 & 0.09 & 0.16 \\
PortScan & 1.00 & 1.00 & 0.98 & 0.99 & 1.00 & 1.00 & 0.98 & 0.99 & 0.99 & 1.00 & 0.86 & 0.92 \\
Web Attack & 1.00 & 0.83 & 0.67 & 0.74 & 1.00 & 0.83 & 0.67 & 0.74 & 1.00 & 0.96 & 0.86 & 0.91 \\
\hline
\textbf{Average} & \textbf{0.99} & \textbf{0.88} & \textbf{0.82} & \textbf{1.00} & \textbf{1.00} & \textbf{0.76} & \textbf{0.88} & \textbf{0.82} & \textbf{0.99} & \textbf{0.94} & \textbf{0.75} & \textbf{0.79} \\
\hline
\end{tabular}%
}
\end{table*}
